Low-Latency Video Conferencing via Optimized Packet Routing and Reordering

In the face of rising global demand for video meetings, managing traffic across geographically distributed (geo-distributed) data centers presents a significant challenge due to the dynamic and limited nature of inter-DC network performance. Facing these issues, this paper introduces two novel techniques, VCRoute and WMJitter, to optimize the performance of geo-distributed video conferencing systems. VCRoute is a routing method designed for audio data packets of video conferences. It treats the routing problem as a Multi-Armed Bandit issue, and utilizes a tailored Thompson Sampling algorithm for resolution. Unlike traditional approaches, VCRoute considers transmitting latency and its variance simultaneously by using Thompson Sampling algorithm, which leads to effective end-to-end latency optimization. In conjunction with VCRoute, we present WMJitter, a watermark-based mechanism for managing network jitter, which can further reduce the end-to-end delay and keep an improved balance between latency and loss rate. Evaluations based on real geo-distributed network performance demonstrate the effectiveness and scalability of VCRoute and WMJitter, offering robust solutions for optimizing video conferencing systems in geo-distributed settings.

==> problem.tex <==
\section{Problem Formulation}\label{sec:problem}

In this section, we formally describe the problem studied in this paper.
Consider a video conferencing system which has $N$ servers deployed in multiple geo-distributed DCs to host audio/video meeting calls. Each meeting session is assigned with one server as the endpoint. All participants of the meeting communicate with the endpoint to send and receive data packets (refer to Figure~\ref{fig:latency:time}). 
As shown in Section~\ref{sec:bg}, it is sometimes more favorable to relay data packets via other servers to obtain better end-to-end latency and users' QoE. Thus, we study the \emph{packet routing problem} in the overlay network composed by the $N$ servers to optimize video conferencing latency and quality.
When a packet arrives at the receiver's side, it is first stored in a jitter buffer to solve the \emph{out-of-order problem} caused by network variation and jitter. 
The out-of-order problem not only affects packet loss rates but also the end-to-end latency. 
Thus, we need to coordinately consider the above two problems to optimize the overall system latency while guaranteeing users' QoE.
For simplicity, we assume that the network bandwidth is not the bottleneck and packets traveling on the network can successfully arrive at receivers.

\textbf{Packet routing.}
In a meeting session, the data packets between users and the endpoint are routed individually. %Thus, in the following, we define the routing problem considering a single packet.
Given a data packet $i$, denote $P_i$ as the routing path of the packet, where $P_i$ is a list of relays with the sender and receiver nodes as the first and last elements in the list. 
We use $Ts$ to denote the timestamp when a packet is generated, $Ta$ as the time when the packet is arrived at receiver's end and $To$ as the time when the packet is out from the jitter buffer. 
\emph{Existing routing methods mainly focus on reducing the packet transmitting time}, namely $Ta-Ts$. However, this does not guarantee low end-to-end latency, namely $To-Ts$, due to the latency spent on packet reordering. 

Thus, our goal in this paper is to propose an application-specific routing method, which aims at finding the best routing $P_i$ for each packet $i$ in a meeting session, so that the average end-to-end latency is minimized. Formally, we have:
\begin{eqnarray}
\arg\min_{P_i}\frac{1}{|D|} \cdot\sum_{i\in D}T(i,P_i)
\end{eqnarray}
where $D$ is the set of packets transmitted during the meeting and $T(i,P_i)$ represents the end-to-end latency of packet $i$ when the selected routing path is $P_i$.


\textbf{Packet reordering.}
%Packets travel through the network to arrive at receivers' end. 
Packets that travel through the network are typically out-of-order when they arrive at the receiver due to network jitter.
%Thus, we need a packet reordering mechanism at the receiver's side to order packets according to their timestamps. Packet reordering may lead to packet loss and also adds up additional time to the packet end-to-end latency.
To ensure packets are in the correct order, a packet reordering mechanism based on packet timestamps is necessary at the receiver's end. However, this mechanism can result in packet loss and increased end-to-end latency for the packets.
%Assume that the network protocol can guarantee successful arrival of all packets and we only focus on the packet loss caused by packet reordering.
Denote the set of packets that are discarded during the reordering process as $D'$. Then the average packet loss rate during the meeting session can be calculated as $r=\frac{|D'|}{|D|}$.
Our goal in this problem is to design a good packet reordering mechanism that can guarantee users' QoE requirements with low added overhead. That is, $r<L$, where $L$ is the user-defined constraint on packet loss rate. 

% Watermarking is a technique used in streaming data processing to track the progress of data processing and ensure that data is processed in a timely and accurate manner. A watermark is a timestamp that represents the latest possible arrival time of an event. In other words, a watermark defines a threshold or deadline for when all data related to a particular window of time must be processed.

% In a streaming processing system, data is received continuously and processed in small batches. A watermark is used to define the end of a batch and the beginning of the next one. This allows the system to track the progress of data processing and ensure that all events within a given window of time are processed before the watermark deadline.

% The watermark is calculated based on the event time of the data being processed. The event time is the time when an event actually occurred, as opposed to the processing time, which is the time when the event is processed. By using event time to calculate the watermark, the system can handle out-of-order events and data delays.

% Watermarking is an important technique in streaming processing because it helps to ensure the accuracy and completeness of results. By defining a deadline for processing data, the system can avoid data loss and ensure that all events within a given time window are accounted for.


\begin{comment}

\begin{CJK*}{UTF8}{gbsn}

对于网络jitter造成的数据包在接收端的丢包问题，我们进行如下的定义。我们的目标是在保障丢包率小于一个给的阈值的情况下，尽可能地降低数据包在接收端的缓存延迟。在一个会议内的一个时间周期$ T $内，丢包率设为$ lr $。设所有时间戳在周期$ T $内，且成功到达接收端的数据包的集合为$ P $。设集合$ P $中，因网络jitter而迟到，且错过输出而被丢弃的包的集合为$ P' $。则丢包率$ lr $可由以下公式定义：
\begin{eqnarray}
lr = \frac{|P'|}{|P|}  
\end{eqnarray}
设数据包集合$ P $的所有数据包的时间戳的集合为$ TS $，所有包在接收端的缓存时间集合为$ BT $，所有包的
丢包率定义为周期$ T $内，到达接收端的包中，因jitter被丢弃的包和到达接收端的所有包的比例。在这里，当到达的包的$ ts $（timestamp）小于$ wm $（watermark）时，包被丢弃。设固定会话时间$ T $内，TS为所有packets的时间戳集合，WM为周期$ T $内的wm（watermark）集合。用$ ts\in TS $，$ wm\in WM $分别表示一个packet的时间戳和watermark。$ Q2(ts,wm) $表示packet是否被丢弃，其中$ ts<wm $时，$ Q2(ts,wm)=1 $表示packet被丢弃；$ ts>=wm $时，$ Q2(ts,wm) =0 $表示packet不被丢弃。目标是对每个ts属于TS，找到最小的wm，使得Q2(ts,wm)的和小于一个给定的阈值。本文采用的watermark更新方式公式如下。
\begin{eqnarray}
wm(i) = ts(i-1)+interval-(jitter+delta)
\end{eqnarray}
其中ts(i-1)为上个到达的packet的时间戳，interval为相邻packet之间的发送间隔，jitter为网络抖动，delta为一个附加的可调旋钮值，根据当前丢包率进行调整。显然，jitter+delta值越大，丢包率越低，但增加的延迟也越大。因此我们的目标是找到满足丢包率的最小jitter+delta值。

\end{CJK*}
\end{comment}

% On arriving at the endpoint, packets in the streams are usually out-of-order and we can sort the packets according to their timestamps to guarantee good user experience. During the sorting, late packets may be dropped to guarantee low latency. For the $i$-th stream, denote the packet loss rate on the route as $lr_i$ and the loss rate caused by packet dropping as $ld_i$. %The total packet loss rate $L_i$ of stream $i$ can be calculated as: 
% % \begin{eqnarray}\label{eq:loss}
% % L_i=1-(1-lr_i)\cdot(1-ld_i) %\nonumber
% % %\\=Lfw_i+Lfp_i-Lfw_i*Lfp_i
% % \end{eqnarray}
% Thus, the numbers of packets of stream $i$ received by endpoints and users during time period $T$ are $Ne_i=(1-lr_i)\cdot(\left \lfloor \frac{T}{t} \right \rfloor +1)$ and $Ns_i=Ne_i\cdot(1-ld_i)$, respectively.


% When a packet is received by the endpoint, it is first put in a buffer and then sorted in a batch. 
% Denote $T_{proc}$ as the time taken for the endpoint to process a received packet. We have $T_{proc}=t_{queue}+O(WlogW)$, where $t_{queue}$ is the queuing delay of the packet and $W$ represents the size of the buffer. $O(WlogW)$ represents the sorting latency.
% Denote the average end-to-end delay of a stream $i$ as $Ts_i$, we have:
% \begin{eqnarray}
% Ts_i=\frac{\sum_{j=0}^{Ne_i-1} T_{route}^j +\sum_{j=0}^{Ns_i-1g} T_{proc}^j}{Ns_i}
% \end{eqnarray}
% where $T_{route}^j$ and $T_{proc}^j$ represent the routing and processing latencies of the $j$-th packet in stream $i$ received by endpoints and users, respectively.


% Given the above formulation, this paper aims to address the \emph{routing problem} by finding a good $list$ for each packet in the streams and address the \emph{out-of-order problem} by designing efficient packet ordering. The goal is to minimize the total packet loss rate of each stream $i$ denoted as $L_i$ while guaranteeing the average packet delay $Ts_i$ is shorter than a predefined constraint $T_{qos}$. Formally, we have:
% \begin{eqnarray}
% \min L_i=1-(1-lr_i)\cdot(1-ld_i)
% \end{eqnarray}
% s.t., \vspace{-2ex}
% \begin{eqnarray}
% Ts_i\le T_{qos}
% \end{eqnarray}

